How Fast Can We Play Tetris Greedily With Rectangular Pieces?

Consider a variant of Tetris played on a board of width $w$ and infinite height, where the pieces are axis-aligned rectangles of arbitrary integer dimensions, the pieces can only be moved before letting them drop, and a row does not disappear once it is full. Suppose we want to follow a greedy strategy: let each rectangle fall where it will end up the lowest given the current state of the board. To do so, we want a data structure which can always suggest a greedy move. In other words, we want a data structure which maintains a set of $O(n)$ rectangles, supports queries which return where to drop the rectangle, and updates which insert a rectangle dropped at a certain position and return the height of the highest point in the updated set of rectangles. We show via a reduction to the Multiphase problem [P\u{a}tra\c{s}cu, 2010] that on a board of width $w=\Theta(n)$, if the OMv conjecture [Henzinger et al., 2015] is true, then both operations cannot be supported in time $O(n^{1/2-\epsilon})$ simultaneously. The reduction also implies polynomial bounds from the 3-SUM conjecture and the APSP conjecture. On the other hand, we show that there is a data structure supporting both operations in $O(n^{1/2}\log^{3/2}n)$ time on boards of width $n^{O(1)}$, matching the lower bound up to a $n^{o(1)}$ factor.

==> Tetris data structure/realated-work.tex <==
Tetris, created in 1984 by Alexey Leonidovich Pajitnov of the  Dorodnitsyn Computing Centre of the Soviet Academy of Science, was one of the greatest inventions of the USSR, one that was widely embraced by the citizens of both the Warsaw Pact and NATO as well as non-aligned countries.
In the computer science literature, the allure of Tetris has been irrepressible, with works using Tetris found in virtually every subdiscipline.

One might be tempted to begin reviewing the literature with the paper whose title is the one single word ``Tetris''  \cite{DBLP:journals/corr/abs-1811-08614}. 
However, one will quickly realize that the Tetris that they speak of is not the game so beloved by humanity, but rather ``Tetris is an Asynchronous Byzantine Fault Tolerance consensus algorithm designed for next generation high-throughput permission and permissionless blockchain.'' 
In continuing though the literature, one quickly realizes that the name ``Tetris'' has been appropriated mercilessly to entitle and describe things that are not directly about the famed game, but are either meant to invoke the idea of putting pieces together or are just an acronym that the authors found cute, no doubt in the hopes that a small fraction of the shine of the real and true Tetris might befall upon their work \cite{
    DBLP:conf/mig/AdamsonBMSJKT14,
    DBLP:conf/iticse/Black17,
    DBLP:journals/adcm/CasazzaP14,
    DBLP:journals/biosystems/Cowley19,
    DBLP:journals/corr/DoblerR17,
    DBLP:journals/dam/GalliSS01,
    DBLP:conf/asplos/GaoPYHK17,
    DBLP:conf/scopes/GoensKCHSH17,
    DBLP:conf/uss/0001DKBCPH20,
    DBLP:conf/isaac/KutylowskiW97,
    DBLP:journals/tmi/LeePPGS19,
    DBLP:conf/icpp/LiWFHTLL16,
    DBLP:conf/iwqos/LingYWY16,
    DBLP:conf/nana/LiuST21,
    DBLP:conf/iccad/LuWLYL18,
    DBLP:journals/jct/Lupini17,
    DBLP:journals/corr/abs-1811-06841,
    DBLP:conf/gvd/Markl98,
    DBLP:conf/icde/MarklZB99,
    DBLP:conf/sigcse/Schocken17,
    DBLP:conf/mass/StaffordRWCAD17,
    DBLP:conf/eurosys/TumanovZPKHG16,
    DBLP:conf/dac/WestZDFKCW19,
    DBLP:journals/tc/WestZDKFCW20,
    DBLP:conf/chiir/Wilson17,
    DBLP:conf/lctrts/XuT07,
    DBLP:journals/taco/XuT09,
    DBLP:conf/IEEEcloud/ZhangRECSWP11}.
Perhaps the most useful of the Tetris-inspired research has been the creation of a floor-cleaning robot which is hinged and can change shape to various Tetris pieces \cite{DBLP:conf/icra/PrabakaranEPN17,
%DBLP:books/mk/GrayR93,
    DBLP:journals/sensors/LePSM18,
    DBLP:journals/access/PrabakaranEPV18}.

As for the game itself, the most research in the computer science community, unsurprisingly, is about getting computers to play Tetris.
There, Tetris has been used as a research tool more often than any other video game \cite{DBLP:journals/ets/Pinnell15} and has been subjected to just about every machine learning and artificial intelligence paradigm %\cite{DBLP:journals/corr/abs-1905-01652}.
\cite{DBLP:journals/corr/abs-1905-01652,
    DBLP:conf/lwa/BohmKM04,
    DBLP:conf/cig/Boumaza09,
    DBLP:conf/gecco/Boumaza11,
    DBLP:conf/ae/Boumaza11,
    DBLP:conf/bracis/SilvaP17,
    DBLP:conf/nips/GabillonGS13,
    DBLP:conf/gecco/GillespieGS17,
    DBLP:conf/cogsci/GittelsonLSG14,
    DBLP:conf/esann/GrossFS08,
    DBLP:conf/gecco/JaskowskiSLK15,
    DBLP:conf/atal/KnoxS10a,
    DBLP:conf/cec/LangenhovenHE10,
    DBLP:journals/sensors/LePSM18,
    DBLP:conf/icml/LichtenbergS19,
    DBLP:conf/dcai/Marin-LoraCS21,
    DBLP:journals/corr/abs-2004-00377,
    DBLP:conf/cig/Muller-Brockhausen21,
    DBLP:conf/iconip/Phon-Amnuaisuk14,
    DBLP:conf/inns-wc/Phon-Amnuaisuk14,
    DBLP:conf/kes/Phon-Amnuaisuk15,
    DBLP:conf/nafips/PickeringC20,
    DBLP:conf/flairs/RomdhaneL08,
    DBLP:conf/setn/RovatsouL10,
    DBLP:journals/jmlr/Scherrer13,
    DBLP:journals/jmlr/ScherrerGGLG15,
    DBLP:conf/gecco/Schrum18,
    DBLP:conf/iclp/SchullerW15,
    DBLP:conf/cogsci/SibertG17,
    DBLP:conf/cogsci/SibertGL15,
    DBLP:journals/neco/SzitaL06,
    DBLP:conf/gi/Thanh16,
    DBLP:conf/annpr/ThiamKS14,
    DBLP:phd/hal/Thiery10,
    DBLP:journals/icga/ThieryS09,
    DBLP:journals/ria/ThieryS09,
    DBLP:journals/icga/ThieryS09a} 
    including, of course, ant colonies \cite{DBLP:conf/gecco/ChenWWSG09}.
However, success is far from guaranteed, as \emph{The Unsuitability of Supervised Backpropagation Networks for Tetris} shows \cite{DBLP:journals/aans/LewisB15}.


Researchers have discovered that in addition to computers, humans can also play Tetris. They have studied how humans interact as they play Tetris and how this relates to primate socialization in general, observing that  ``baboon social intelligence contrasts both with that of Tetris players and human infants, because both have the ability to provoke epistemic effects'' \cite{DBLP:journals/connection/CowleyM06}.
Other human angles have been studied as well, including 
studying styles of play \cite{DBLP:conf/cogsci/BerryG19,DBLP:conf/hicss/KeatingLTH17}, humanity's suboptimal choices \cite{DBLP:conf/cogsci/SibertG19}, eye movement while playing \cite{DBLP:conf/bcshci/JermannNL10,DBLP:conf/icmi/LiNJ10,
DBLP:conf/mmsp/LiNJ11,DBLP:conf/chiplay/SpielBK19},
and how champion Tetris players play, including the relationship between Hick’s Law and expertise \cite{DBLP:conf/cogsci/LindstedtG20}, and social exertion \cite{DBLP:conf/intetain/MastV16}.
Tetris has been used as well to develop a model of cognition \cite{DBLP:conf/iccm/VekslerG04}.
Additionally, a ``Brain Computer Interface (BCI) game that is inspired [by] the Tetris game'' was created where they perform experiments with children with attention deficit and hyperactivity disorder (ADHD) \cite{DBLP:conf/segah/PiresTCNC11} (see also \cite{DBLP:conf/icmi/KrolFZ17,DBLP:conf/um/PatsisSVT13}).

    
Several kinds of researchers have worked on helping humans to play Tetris better \cite{DBLP:conf/acg/OikawaHI19} and addressed the all-important work on the influence of the tempo of the music one listens to while playing Tetris on the score
 \cite{DBLP:conf/cig/HufschmittCJ20,DBLP:conf/chiplay/HufschmittCJ20,DBLP:conf/iui/HufschmittCJ21}.
Other researchers worked to study human performance in Tetris, including the elements that can be used to predict whether a human will become a Tetris master \cite{DBLP:conf/cosecivi/Ariza15,
DBLP:conf/cogsci/GrayPLSJMAA14,
DBLP:conf/cogsci/LindstedtG13,
DBLP:conf/cogsci/SibertGL15,
DBLP:conf/cogsci/SibertLG14}.
The issue of dynamically adjusting the difficulty of the game has also been the subject of study \cite{
DBLP:conf/iccbr/ArizaSG17,
DBLP:conf/iccbr/ArizaSG19,
DBLP:conf/cosecivi/LoraSG16,
DBLP:conf/flairs/LoraSGG16,
DBLP:conf/chi/SpielBK17}.



One great step in the development of Tetris was the creation of a mobile version of ``the stable and reliable game based on the mature game algorithm'' \cite{DBLP:conf/icica/WangCL11}. 
Also of note was  \emph{Pop-out Tetris}
\cite{DBLP:conf/jcsse/KongsilpCK18} where they applied the ``Fish Tank Virtual Reality technique to a commodity tablet'' as well as an embedded system created for Tetris \cite{DBLP:conf/csreaESA/PangPT10}. The long history of Tetris and its many implementations has led one group to study these implementations over time, deeming them ``worthy of historical analysis'' \cite{DBLP:conf/digra/Jordan09}.
    
From an education perspective, Tetris was used by \cite{DBLP:conf/digitel/Chen10} to help students learn Chinese proverbs by putting Chinese characters on each Tetris block. 
Within mainstream computer science education, Tetris is a common subject of programming projects
    \cite{DBLP:journals/sigcse/Parlante01}.

 Tetris has also spawned its own fan fiction, which has been studied: ``In [one work] there are also racial and gender complications, the story ending on a humorous note with an absurd twist, as in a Samuel Beckett play, when a message appears over the head of the disillusioned blocks: `Play again?'. It is obvious that in these stories the game of Tetris is an allegory for human life and behavior'' \cite{DBLP:conf/digra/RambuschSEW09}.
 From the point of view of a narrative, ``An experiment was made with the game  Tetris,  showing  that  a  control  system designed  around  evaluation  of  player’s  tension [makes] it possible to obtain an execution trace [close] to a narrative one'' \cite{DBLP:journals/ijigs/DelmasCA08}.


Following the immense success of cannabis legalization, Tetris has followed suit with Enhanced Tetris Legalization 
\cite{DBLP:conf/pci/DadaliarisNKOLS16,
DBLP:conf/seeda/DadaliarisNOHTA16,
DBLP:journals/jolpe/DadaliarisOKNHG17,
DBLP:conf/mocast/OikonomouDLKS18}.



A surprisingly active field has been the ability of a Tetris player to  hide messages via gameplay \cite{DBLP:conf/icmlc/OuC11,DBLP:journals/isci/OuC14,DBLP:journals/iet-ipr/SuCLY20,DBLP:journals/iet-ipr/X21}.

On the more theoretical side,
it has been shown how to view the game through the lens of Krohn-Rhodes theory \cite{DBLP:journals/corr/abs-2004-09022},
how to use mixed integer programming to pack Tetris-like pieces in 3D \cite{DBLP:journals/4or/Fasano04},
 how to create Tetris boards with a given pattern \cite{DBLP:journals/ijigs/HoogeboomK04}, 
 and how to generate polyominoes \cite{DBLP:journals/endm/FormentiM17}.
 In \cite{DBLP:journals/dm/BaccheriniM08}, they
 ``propose a straight Coward algorithm to transform a Tetris-like game into its corresponding automaton.'' 
 
 
 Closer to the topic of this paper is the algorithmic work relating to the complexity of playing Tetris.
 The starting point for this consists of results about the hardness of approximating various Tetris objectives (e.g.~number of rows cleared, number of moves before reaching a certain height), even with foreknowledge of the entire sequence of pieces \cite{DBLP:journals/ijcga/BreukelaarDHHKL04,
    DBLP:journals/corr/cs-CC-0210020,
    DBLP:conf/cocoon/DemaineHL03}.
This work was generalized to show $\NP$-completeness for $k$-ominos with $k\geq 4$, and surprisingly also show that it is $\NP$-complete to clear the board even for $k=2$ when rotations are not allowed \cite{DBLP:journals/jip/DemaineDEHLLY17}.
These reductions were further tightened in \cite{DBLP:journals/jip/AsifCDDHLS20,DBLP:journals/corr/abs-2009-14336} to when the board is small and in \cite{DBLP:journals/corr/Temprano15} for the variant where you can rotate and then move down, but when no rotations are allowed after the block has begun to fall.
The undecidability of whether a set of sequences of Tetris moves described by a regular language contains a sequence that results in an empty board has been proven \cite{DBLP:journals/ipl/HoogeboomK04}.
While this all sounds very negative, a more positive outlook can be found in \emph{Why Most Decisions Are Easy in Tetris} \cite{DBLP:conf/icml/SimsekAK16}.
          
Unrelated to Tetris, the problem studied is a form of dynamic \emph{reverse range query} \cite{DBLP:journals/entcs/Takaoka03}. In a standard range query one has a collection of objects which are preprocessed such that given a range, some question about the objects that intersect the range can be answered. The literature on range queries is immense, with variants depending on the type of objects, the type of ranges, and the specific queries (see, for example, the chapter on range queries in \cite{DBLP:reference/cg/2004}). Classically, what is interesting is that for points and queries that ask how many points intersect the range, the answer is polylog for orthogonal queries and polynomial for non-orthogonal queries, assuming reasonable space.  
In a reverse range query, we are looking for the ranges that would give a certain result, and to provide the extreme such range under some measure; if there is only a single such reverse range query without parameters, this is interesting as a data structure only when the point set is changing dynamically.

For example, the classic problem of finding the smallest circle enclosing a set of points in the plane can be viewed as such a reverse range query, where one is searching for a circular range query that returns $n$ points, and among all such queries is looking for the smallest one; in the dynamic case the best known data structure takes polylogarithmic time, even when deletions are allowed \cite{DBLP:journals/dcg/Chan20a}. 
On the other hand, the best known data structure for maintaining the largest empty circle in a set of points (with center constrained to be inside a fixed triangle) takes time $\tilde{O}(n^{7/8})$ \cite{DBLP:journals/siamcomp/Chan03} (or $\tilde{O}(n^{11/12})$ when deletions are also allowed \cite{DBLP:journals/dcg/Chan20a}). 

For the case of finding (not necessarily axis-aligned) rectangular ranges enclosing all points, the best known data structure takes time $\tilde{O}(n^{1/2})$ to find the minimum-perimeter range and  $\tilde{O}(n^{5/6})$ for the minimum-area range (also \cite{DBLP:journals/siamcomp/Chan03}).
No conditional lower bounds are known for these problems, which remains a major open problem.
In our case we are looking for a three-sided upwards-facing query that returns zero objects,\footnote{Although we have presented our results as a board containing rectangles, our upper and lower bounds also hold for points.} and among all such queries to find the one that is as low as possible.  
